FourierGNN: Rethinking Multivariate Time Series Forecasting from a Pure Graph Perspective

Multivariate time series (MTS) forecasting has shown great importance in numerous industries. Current state-of-the-art graph neural network (GNN)-based forecasting methods usually require both graph networks (e.g., GCN) and temporal networks (e.g., LSTM) to capture inter-series (spatial) dynamics and intra-series (temporal) dependencies, respectively. However, the uncertain compatibility of the two networks puts an extra burden on handcrafted model designs. Moreover, the separate spatial and temporal modeling naturally violates the unified spatiotemporal inter-dependencies in real world, which largely hinders the forecasting performance. To overcome these problems, we explore an interesting direction of directly applying graph networks and rethink MTS forecasting from a pure graph perspective. We first define a novel data structure, hypervariate graph, which regards each series value (regardless of variates or timestamps) as a graph node, and represents sliding windows as space-time fully-connected graphs. This perspective considers spatiotemporal dynamics unitedly and reformulates classic MTS forecasting into the predictions on hypervariate graphs. Then, we propose a novel architecture Fourier Graph Neural Network (FourierGNN) by stacking our proposed Fourier Graph Operator (FGO) to perform matrix multiplications in Fourier space. FourierGNN accommodates adequate expressiveness and achieves much lower complexity, which can effectively and efficiently accomplish the forecasting. Besides, our theoretical analysis reveals FGO's equivalence to graph convolutions in the time domain, which further verifies the validity of FourierGNN. Extensive experiments on seven datasets have demonstrated our superior performance with higher efficiency and fewer parameters compared with state-of-the-art methods.

==> 3_method.tex <==
%$x_t^{(n)} \in \mathbb{R}^1$ --> $\bm{x}_t \in \mathbb{R}^{N}$ --> $X_t \in \mathbb{R}^{N \times T}$  -->  $\mathcal{G}({X^\mathcal{G}_t},{A_t^\mathcal{G}})$ --> $\mathcal{G}({\mathbf{X}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> $\mathcal{G}({\mathcal{X}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> Shift Operator (AXW) --> $\mathcal{G}({\mathcal{Y}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> $\mathcal{G}({\mathbf{Y}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> 
%$ \hat{Y}_t \in \mathbb{R}^{N \times \tau}$.
\section{Problem Definition}
%Let us denote an entire multivariate time series (MTS) dataset as $\mathbb{X} \in \mathbb{R}^{N\times L}$ where $N$ is the number of variables and $L$ is the number of timestamps of the whole dataset. 
%Under the rolling setting, the time-series inputs are defined as averagely sampled lookback windows of length $T$, i.e., $\{X|X\subset\mathbb{X},X\in\mathbb{R}^{N\times T}\}$. 
Given the multivariate time series input, i.e., the lookback window $X_t=[\bm{x}_{t-T+1},...,\bm{x}_t]\in\mathbb{R}^{N\times T}$ at timestamps $t$ with the number of variables $N$ and the lookback window size $T$, where $\bm{x} \in \mathbb{R}^{N}$ denotes the multivariate values of $N$ distinct series at timestamp $t$, then the \textit{multivariate time series forecasting} task is to predict the next $\tau$ timestamps $Y_t=[{\bm{x}}_{t+1}, ..., {\bm{x}}_{t+\tau}]\in \mathbb{R}^{N \times \tau}$ based on the historical $T$ observations $X_t=[\bm{x}_{t-T+1},...,\bm{x}_t]$. The forecasting process can be given by:
% \begin{equation}\label{eq:problem_define}
%     \hat{\bm{x}}_{t+1},...,\hat{\bm{x}}_{t+\tau} = {F_{\theta}}(\bm{x}_{t-T+1},...,\bm{x}_t))
% \end{equation}
\begin{equation}\label{eq:problem_define}
   \hat{Y}_t  = {F_{\theta}}(X_t) = {F_{\theta}}([\bm{x}_{t-T+1},...,\bm{x}_t])
\end{equation}
where $\hat{Y}_t$ are the predicted results; the forecasting function is denoted as $F_\theta$ parameterized by $\theta$.
In practice, many MTS forecasting models usually leverage a \textit{graph network} (assume parameterized by $\theta_g$) to learn the spatial dynamics and a \textit{temporal network} (assume parameterized by $\theta_t$)  to learn the temporal dependencies, respectively \cite{zonghanwu2019, Cao2020,Bai2020nips,wu2020connecting,tampsgcnets2022}. Thus, the original definition of Equation (\ref{eq:problem_define}) can be rewritten to:
% \begin{equation}\label{eq:problem_define_gt}
%     \hat{\bm{x}}_{t+1},...,\hat{\bm{x}}_{t+\tau} = {F_{{\theta_g},{\theta_t}}}(\bm{x}_{t-T+1},...,\bm{x}_t)
% \end{equation}
\begin{equation}\label{eq:problem_define_gt}
    \hat{Y}_t  = {F_{\theta}}(X_t) = F_{\theta_g,\theta_t}([\bm{x}_{t-T+1},...,\bm{x}_t])
\end{equation}
where original parameters $\theta$ are exposed to the parameters of the graph network and the temporal network ${\theta_g}, {\theta_t}$ to make predictions based on the learned spatial-temporal dependencies.
%{
%\color{red}
%In the following section, we detnote the lookback window at timestamp $t$ as $X_t$, and the horizon window as $Y_t$ for brevity. 
%}

% $F_{\theta_g}$ with parameters $\theta_g$ for spatial correlations and a temporal network $F_{\theta_t}$ with parameters $\theta_t$ for temporal dependencies. Subsequently, a forecasting function $F_{\theta_f}$ with parameters $\theta_f$ is applied to make predictions based on the learned spatial-temporal dependencies. As a result, the forecasting problem is formulated as follows:
% \begin{equation}
%     \hat{X}_{t+1},...,\hat{X}_{t+\tau} = {F_{\theta_f}}((F_{\theta_g},F_{\theta_s})(X_{t-T},...,X_t))
% \end{equation}
%where $\operatorname{F}$ is the forecasting function and $\Theta$ is the learnable parameters of the forecasting function.


\section{Methodology}
In this section, we elaborate on our new framework: First, we start with our pure graph formulation with a novel data structure for MTS forecasting
in Section \ref{sec:method_pure_graph_form}. Then, we illustrate the proposed neural architecture, Fourier Graph Neural Network (FourierGNN), for this formulation in Section \ref{sec:method_fouriergnn}. Besides, we 
present theoretical analysis towards FourierGNN to demonstrate its validity.

\subsection{The Pure Graph Formulation}\label{sec:method_pure_graph_form}
To overcome the uncertain compatibility of the graph network and the temporal network as aforementioned in Section \ref{sec:intro}, and learn united spatiotemporal dynamics, we introduce a \textit{pure} graph formulation that refines Equation (\ref{eq:problem_define_gt}) by introducing a novel data structure, \textit{hypervariate graph}, for time series.
% In this paper, our goal is to learn an united view of spatiotemporal dynamics simultaneously and model the interdependencies between variables and their evolution over time, to this end, we build a hypervariate graph $\mathcal{G}=(X,A)$ attributed to each $X$ and further formulate the problem of MTS forecasting on the hypervariate graph. 
 \begin{myDef}[\textbf{Hypervariate Graph}]
\label{hypervariate_graph}
    Given a multivariate time series input $X_t \in \mathbb{R}^{N \times T}$ of $N$ variables over $T$ timestamps, we construct a hypervariate graph of $NT$ nodes, $\mathcal{G}_t=({X}^{\mathcal{G}}_t, {A}^{\mathcal{G}}_t)$, by regarding each element of $X_t$ 
    %(regardless of variables or timestamps)
    as one node of $\mathcal{G}_t$ such that ${X}^{\mathcal{G}}_t \in \mathbb{R}^{NT \times 1}$ stand for the node features and ${A}^{\mathcal{G}}_t \in \mathbb{R}^{NT \times NT}$ is the adjacency matrix.
    % variable at each timestamp is represented by a node in the graph, with $X\in \mathbb{R}^{NT}$ representing the nodes and $A \in \mathbb{R}^{(NT) \times (NT)}$ being the adjacency matrix. We refer to the graph $\mathcal{G}$ as a hypervariate graph.
\end{myDef}
 The hypervariate graph $\mathcal{G}_t$ contains $NT$ nodes that represent values of each variable at each timestamp in $X_t$. %and $A^{\mathcal{G}}_t \in \mathbb{R}^{NT \times NT}$ represents the connection structure of $\mathcal{G}.
 Since the prior graph structure is usually unknown in most scenarios, and each element of $X_t$ are spatially or temporally correlated with each other, we assume all nodes in the hypervariate graph $\mathcal{G}_t$ are fully-connected, in order to learn a joint spatiotemporal representation. More analysis about the hypervariate graph can be seen in Appendix \ref{analysis_hypervariate_graph}.
 Accodingly,
 %given the observed values of previous $T$ steps at timestamp $t$, i.e., $X_{t-T+1},...,X_{t}\in \mathbb{R}^{N\times T}$, 
 %the task of \textit{multivariate time series forecasting} is to predict the values of $N$ variables for next $\tau$ steps denoted as $\hat{X}_{t+1},...,\hat{X}_{t+\tau}\in \mathbb{R}^{N\times \tau}$ on the hypervariate graph $\mathcal{G}$. 
 %Thus, the problem formulation is modified as follows:%according to the learned spatial-temporal dependencies 
 we reformulate \textit{multivariate time series forecasting} into the predictions on the hypervariate graphs and rewrite the equation (\ref{eq:problem_define_gt}) as:
 %on the hypervariate graph $\mathcal{G}_t=({X}^{\mathcal{G}}_t, {A}^{\mathcal{G}}_t)$ and the problem formulation is modified as follows:
\begin{equation}
    \hat{Y}_t =F_{\theta_\mathcal{G}}({X^\mathcal{G}_t},{A_t^\mathcal{G}})
\end{equation}
where $\theta_\mathcal{G}$ stand for the parameters of hypervariate graphs,
instead of  being split into separate ${\theta_g}$ and ${\theta_t}$ for two networks in Equation (\ref{eq:problem_define_gt}).
With such a formulation, we can view the spatial dynamics and the temporal dependencies with an united structure, which benefits modeling the real-world spatiotemporal inter-dependencies.


%where $\operatorname{F}$ is the forecasting model with parameters $\Theta$. 

\subsection{FourierGNN}\label{sec:method_fouriergnn}
%With the hypervariate graph $\mathcal{G}$, we can view spatiotemporal dynamics as a whole, which facilitates the modeling of intricate interdependencies between various variables and timestamps. 
%To learn the united spatiotemporal dynamics, we perform graph convolutions on $\mathcal{G}$.
%Nevertheless, 
Though the pure graph formulation enhances spatiotemporal modeling, 
the order and size of hypervariate graphs increase with the number of variables $N$ and the length of window $T$, which makes classic graph networks (e.g., GCN~\cite{}, GAT~\cite{}, etc) computationally expensive (usually quadratic complexity) and suffer from optimization difficulties to obtaining accurate hidden node representations~\cite{}. 
In this regard, we propose an efficient and effective method, FourierGNN, for the pure graph formulation. Specifically, we first elaborate on our proposed built-in component, Fourier Graph Shift Operator (FGSO) in Section \ref{FGSO}; then we illustrate the stacked architecture of FourierGNN with FGSOs 
in Section \ref{FGNN}; finally, we present the overall pipeline using FourierGNN for forecasting in Section \ref{architecture}.



% Specifically, in \ref{FGSO} we design a replacement of classic graph convolution units in Fourier space (i.e., FGSO), and then implement graph convolutions by stacking FGSOs in Fourier space (i.e., FourierGNN) in \ref{FGNN}. Finally, we introduce our overall network architecture based on FourierGNN for MTS forecasting in \ref{architecture}.

%FourierGNN we introduce  shift operator, in Section XXX, 
%built on operator, we illustarte archir3ecture, Figure ref{},
%we theoreatical analysis  
%4.2.1 shift operator (including inference for FGSO)
%4.2.2 overall architecture (current 4.2.1 + partial current 4.2.3)
%4.2.3 model analysis (prove in 4.2.3)

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/FourierGNN_new.pdf}
    \caption{\textcolor{red}{The network architecture of our proposed model}. Given an input $X\in \mathbb{R}^{N \times T}$, we 1) embed $X$ into $\mathbf{X}\in \mathbb{R}^{N\times T \times d}$; 2) transform $\mathbf{X}$ to Fourier space $\mathcal{X} \in \mathbb{C}^{N \times T \times d}$ by 2D DFT on the discrete N × T spatial-temporal space; 3) perform graph convolutions in Fourier space by conducting multiplication of FGSO $\mathcal{S}$ and $\mathcal{X}$ in the $K$-layer FourierGNN; 4) transform the output of FourierGNN to time domain $\mathbf{X}_{\Psi}\in \mathbb{R}^{N\times T \times d}$ by 2D IDFT; 5) generate $\tau$-step predictions $\hat{X} \in \mathbb{R}^{N \times \tau}$ via feeding $\mathbf{X}_{\Psi}$ to a two-layer feed-forward network.}
    \label{fig:model_fig}
\end{figure}

\subsubsection{Fourier Graph Shift Operator}\label{FGSO}
According to the discrete signal processing on graphs \cite{SandryhailaM13}, a graph shift operator (GSO) is defined as a general family of operators which enables the diffusion of information over graph structures~\cite{GamaRB20,Dasoulas2021}.

%Note that the supra-graph $n=NT$.


\TODO{
Definition 2 --> 
(4) --> 
However, Equation (4) has quadratic complexity due to S X ~ n, which brings potential challenges in our pure graph formulation. 
Thus, we define a Fourier Graph shift operator to solve this problem. 

-->
Definition 3,  $\mathcal{S}$ = 

-->



}


\begin{myDef}[\textbf{Graph Shift Operator}]
\label{def:gso}
Given a graph $G$ with $n$ nodes, a matrix $S\in\mathbb{R}^{n\times n}$ is called a \textit{Graph Shift Operator} (GSO) if it satisfies $S_{ij}=0$ if $i\neq j$ and nodes $i,j$ are not connected.
\end{myDef}
Usually, the graph shift operator includes the adjacency, Laplacian matrices and their according normalization as instances of its class~\cite{}. 
Thus, given the graph $G$ attributed to $X\in\mathbb{R}^{n\times d}$ and the graph shift operator $S$, %a general form of spatial-based graph convolution is defined as
we can express the classic graph convolution~\cite{KipfW17} as:
%a general form of graph convolution~\cite{KipfW17} is defined as
\begin{equation}
\label{equ:graph_covolution}
    O({X}):=S{X}{W}
\end{equation}
with the parameter matrix ${W}\in\mathbb{R}^{d\times d}$. Regarding $S$ as $n\times n$ scores, we can define a matrix-valued kernel $\kappa: [n]\times [n] \xrightarrow{} \mathbb{R}^{d\times d}$ with $\kappa[i,j]=S_{ij}\circ {W}$, where $[n]=\{1,2,\cdots,n\}$. Then the graph convolution can be viewed as a kernel summation:
\begin{equation}
    O({X})[i]=\sum_{j=1}^n {X}[j]\kappa[i,j]  \quad\quad   \forall i \in [n].
\end{equation}
In the special case of the Green's kernel $\kappa[i,j]=\kappa[i-j]$, we can rewrite the above equation as:
\begin{equation}\label{equ:kernel_summation}
    O({X})[i]=\sum_{j=1}^n {X}[j]\kappa[i-j]=(X*\kappa)[i]  \quad\quad   \forall i \in [n].
\end{equation}
with $X*\kappa$ denotes the convolution of discrete sequences $X$ and $\kappa$. According to the convolution theorem~\cite{1970An} (see Appendix \ref{convolution_theorem_appendix}), we can rewrite the graph convolution of Equation (\ref{equ:kernel_summation}) as:
\begin{equation}
\label{equ:fno}
O(X)(i) = \mathcal{F}^{-1}\left(\mathcal{F}(X)\mathcal{F}(\kappa)\right)(i)\quad\quad  \forall i \in [n].
\end{equation}
where $\mathcal{F}$ and $\mathcal{F}^{-1}$ denote the Discrete Fourier Transform (DFT) and the inverse DFT, respectively. 
%The multiplication in the Fourier space is a lower-complexity computation compared to the graph convolution, and DFT can be efficiently implemented by the fast Fourier transform (FFT). %In the following, we define the Fourier Graph Shift Operator.
\begin{myDef}[\textbf{Fourier Graph Shift Operator}]
\label{def:fgso}
Given a graph $G=(X, S)$ with input $X\in\mathbb{R}^{n\times d}$ and GSO $S \in\mathbb{R}^{n\times n}$ and the weight matrix $W\in\mathbb{R}^{d\times d}$, we reformulate the graph convolution as:
\begin{equation}
    \label{equ:fgso}
    \mathcal{F}(SXW)=\mathcal{F}(X)\times_n\mathcal{F}(\kappa)
\end{equation}
%where we define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).
where $\mathcal{F}$ denotes DFT, satisfies $\kappa[i,j]=\kappa[i-j]$, and $\times_n$ is matrix multiplication on dimensions except that of $n$. We define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).
\end{myDef} 
In particular, turning to our case of the fully-connected hypervariate graph $\mathcal{G}$ with a fully-connected GSO $A^{\mathcal{G}}_t\in\{1\}^{n \times n}$, it yields the space-invariant kernel $\kappa[i,j]=A^{\mathcal{G}}_{ij}\circ{W}=W$ and $\mathcal{F}(A^{\mathcal{G}}_tX^{\mathcal{G}}_tW)=\mathcal{F}(X^{\mathcal{G}}_t)\mathcal{F}(\kappa)$. Accordingly, we can parameterize FGSO $\mathcal{A}^{\mathcal{G}}_t$ with a complex-valued matrix $\mathbb{C}^{d \times d}$ which is frequency-invariant and is computationally low costly compared to a varying kernel resulting a parameterized matrix of $\mathbb{C}^{n \times d\times d}$. 
%Furthermore, we generalize Definition \ref{def:fgso} to 2D discrete space, i.e., from $[n]$ to $[N]\times[T]$, corresponding to the finite discrete spatio-temporal space of multivariate time series. 
See Appendix \ref{explanation} for more explanations on the frequency-invariant FGSO. 
%and the extension to 2D domain.

\textbf{Remarks}. 
%Compared with FGSO and FNO, frequency-invariant FGSO has several advantages. 
Frequency-invariant FGSO has several advantages. 
Assume a graph with $n$ nodes and the embedding dimension $d$ ($d\leq n$). 1) \textit{Efficiency}: the time complexity of frequency-invariant FGSO is $O(nd\operatorname{log}n+nd^2)$ for DFT, IDFT and the matrix multiplication compared with that of $O(n^2d+nd^2)$ on a GSO. 2) \textit{Scale-free parameters}: frequency-invariant FGSO strategically shares $O(d^2)$ parameters for each node and the parameter volume is agnostic to the data scale.
%, while the parameter count of FNO is $O(nd^2)$.% More analyses are given in Appendix \ref{proof_proposition}.

\subsubsection{Fourier Graph Neural Networks}\label{FGNN}

\TODO{ 
The specific design of  FourierGNN is by stacking multiple layers of  GGSOs with learnable layers. Specifically, we can define FourierGNN as: 

$ \operatorname{FourierGNN}(X, \mathcal{S}) = \mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\times_n\mathcal{S}_{0:k}\right)\quad s.t.\  \mathcal{S}_{0:k}=\mathcal{S}_0\times_n\cdots\mathcal{S}_{K-1}\times_n\mathcal{S}_{K} $
}
where $S =$






Graph filters as core operations in graph signal processing are linear transformations expressed as polynomials of the graph shift operator~\cite{isufi2021edgenets,MateosSMR19} and can be used to exactly model graph convolutions and capture multi-order diffusion on graph structures~\cite{SegarraMMR17}. 
%\begin{equation}
%    Z_k = S^{K:0} Z_{k-1} W^{K}
%\end{equation}
The $K$-order graph filters $H_K$ are defined as follows~\cite{isufi2021edgenets,SegarraMMR17}:
%graph filter-->edge varying graph filter
\begin{equation}
    H_{K} X= S_0X+S_1S_0X+...+S_KS_{K-1}...S_0X=\sum_{k=0}^{K}\left ( \prod_{k'=0}^{k} S_{k'} \right ) X
\end{equation}
where $S_0$ denotes the identity matrix, $\{S_k\}_{k=1}^K$ is a collection of $K$ GSOs sharing the sparsity pattern of $S$, and $S_k\in\mathbb{R}^{n\times n}$ corresponds to the $k$-th diffusion step.
%\begin{equation}
%    X^(k) = S_K X^(k-1)
%\end{equation}
To capture the time-varying counterparts, we design edge-variant graph filters $H_{K}^{EV}$ by adopting different weights to measure the information of different neighbors in each diffusion order~\cite{isufi2021edgenets}:
%the edge-variant graph filters $H_{EV}$ are defined as follows~\cite{isufi2021edgenets,SegarraMMR17}: given GSO $S\in\mathbb{R}^{n\times n}$ corresponding to a graph with $n$ nodes,
\begin{equation}
    H_{K}^{EV} X = S_0 X W_0+S_1(S_0XW_0)W_1+...+S_K(S_{K-1}...(S_0XW_0)...W_{K-1})W_K %=\sum_{k=0}^{K}S_{k:0}
\end{equation}
%\begin{equation}
%   X_K= \Phi_K X_{K-1} W_{K}
%\end{equation}
%where $S_0$ denotes the identity matrix, $\{S_k\}_{k=1}^K$ is a collection of $K$ edge-weighting GSOs sharing the sparsity pattern of $S$, and $S_k\in\mathbb{R}^{n\times n}$ corresponds to the $k$-th diffusion step. 
where $W_{k} \in \mathbb{R}^{d \times d}$ is a parameter matrix that affords flexibility to process different features with different filter parameters.
The edge-variant graph filters are proved effective to yield a highly discriminative model and lay the foundation for the unification of GCNs and GATs~\cite{isufi2021edgenets}. We further extend Equation (\ref{equ:fgso}) to $H^{EV}_K$ and reformulate the multi-order graph convolution in a recursive form.
%, where we omit the weight $W$ for conciseness.
%\prod_{i=1}^k S_{i}
\begin{myPro}%[\textbf{Equivalence}]
\label{pro:filter}
Given a graph input $X\in\mathbb{R}^{n\times d}$, the $K$-order graph convolution under the edge-variant graph filter $H^{EV}_K$
%=\sum_{k=0}^{K}A_{k:0}$ with $\{A_k\in\mathbb{R}^{n\times n}\}_{k=0}^K$ 
is reformulated as follows:
    \begin{equation} 
    \label{equ:fgso_filter}
        H_K^{EV}X=\mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\times_n\mathcal{S}_{0:k}\right)\quad s.t.\  \mathcal{S}_{0:k}=\mathcal{S}_0\times_n\cdots\mathcal{S}_{K-1}\times_n\mathcal{S}_{K}
    \end{equation}
where $\mathcal{S}_k\in\mathbb{C}^{n\times d\times d}$ is the $k$-th FGSO satisfying $\mathcal{F}(S_k {X} W_k)=\mathcal{F}({X})\times_n\mathcal{S}_k$, $\mathcal{S}_0$ is the identity matrix, and $\mathcal{F}$ and $\mathcal{F}^{-1}$ denote the discrete Fourier transform and its reverse, respectively.
\end{myPro}
Proposition \ref{pro:filter} proved in Appendix \ref{sec:filter} states that we can rewrite the multi-order graph convolution corresponding to $H_K^{EV}$ as a summation of a recursive multiplication of individual FGSO in Fourier space. Corresponding to our case of the hypervariate graph $\mathcal{G}$, we can similarly adopt $K$ frequency-invariant FGSOs and parameterize each FGSO $\mathcal{A}_k$ with a complex-valued matrix $\mathbb{C}^{d\times d}$. This saves a large amount of computation costs and results in a concise form:
\begin{equation} 
    \label{equ:fgso_filter_2}
        H_K^{EV}X=\mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\mathcal{A}_{0:k}\right)\quad s.t.\  \mathcal{A}_{0:k}=\prod_{i=0}^k\mathcal{A}_i
    \end{equation}
The recursive composition has a nice property that $\mathcal{A}_{0:k}=\mathcal{A}_{0:k-1}\mathcal{A}_k$, which inspires us to design a complex-valued feed forward network with $\mathcal{A}_k$ being the complex weights for the $k$-th layer. However, both the FGSO and edge-variant graph filter are linear transformations, limiting the capability of modeling non-linear information diffusion on graphs. Following by the convention in GNNs, we introduce the non-linear activation and biases to reformulate the $k$-the layer as follows: 
\begin{equation}
    \label{equ:layer}
    \mathcal{X}_k = \sigma(\mathcal{X}_{k-1}\mathcal{A}_k+b_k)
\end{equation}
with the complex weight $\mathcal{A}_k \in \mathbb{C}^{d\times d}$, biases $b_k \in \mathbb{C}^{d}$ and the activation function $\sigma$. Accordingly, we design a Fourier graph neural network (FourierGNN) in Fourier space according to Equations (\ref{equ:fgso_filter}) and (\ref{equ:layer}), as shown in Fig. \ref{fig:model_fig}. Accordingly, the $K$-layer FourierGNN $\Psi_K$ is formulated:
\begin{equation}
    \Psi_K(\mathcal{X})=\sum_{k=0}^K \mathcal{X}_{k} \quad s.t.\ \mathcal{X}_k=\sigma(\mathcal{X}_{k-1}\mathcal{A}_k+b_k)
\end{equation}
where $\mathcal{X}_0:=\mathcal{F}(\mathbf{X})$, $\{\mathcal{A}_k\in\mathbb{C}^{d\times d}\}_{k=1}^K$ and $\{b_{k}\in\mathbb{C}^{d}\}_{k=1}^K$ are complex-valued parameters. 
%The frequency output $\Psi_K(\mathcal{X})$ is then transformed via IDFT, followed with feed forward networks (see Appendix \ref{subsec:es} for more details) to make multi-step forecasting in the time domain.

\textbf{Remarks}. FourierGNN efficiently learns edge- and neighbor-dependent weights to compute multi-order graph convolutions on one fly in Fourier space with scale-free parameter volume. For $K$ iterations of graph convolutions, GCNs have a general time complexity of $O(Kn^2d+Knd^2)$, 
%and FNO needs $O(Knd\operatorname{log}n+Knd^2)$, 
and FourierGNN achieves a time complexity of $O(nd\operatorname{log}n+Knd^2+Knd)$. 
FourierGNN 
%saves time costs from FNO in Fourier transforms and 
is much more efficient than GCNs, especially in our case with $n=NT$ for a given raw input $X^{\mathcal{G}}_t\in\mathbb{R}^{N\times T}$. 
See Appendix \ref{compares} for more details about the relations and differences between FourierGNN with other neural networks.
%FNO, adaptive FNO, and GNNs.

% to connect all observed values $\{x_{it}\}$ among variables and timestamps
\subsubsection{Overall Architecture} \label{architecture}
\label{sec:ovarc}
The overall architecture of our model is illustrated in Fig. \ref{fig:model_fig}. Given the MTS input data $X_t \in \mathbb{R}^{N\times T}$, first we construct a fully-connected hypervariate graph $\mathcal{G}=(X^{\mathcal{G}}_t, A^{\mathcal{G}}_t)$ with $X^{\mathcal{G}}_t \in \mathbb{R}^{NT \times 1}$. Then, we embed the data into embeddings $\mathbf{X}^{\mathcal{G}}_t \in \mathbb{R}^{NT\times d}$ by assigning a $d$-dimension vector for each node using an embedding matrix $E_\phi\in\mathbb{R}^{1\times d}$, i.e., $\mathbf{X}^{\mathcal{G}}_t=X^{\mathcal{G}}_t \times E_\phi$. 
%Instead of directly learning the huge embedding matrix, we introduce two small parameter matrices: 1) a variable embedding matrix $\phi_v\in\mathbb{R}^{N\times 1\times d}$, and 2) a temporal embedding matrix $\phi_u\in\mathbb{R}^{1\times T\times d}$ to factorize $\Phi$, i.e., $\Phi=\phi_v\times \phi_u$. 

Subsequently, we perform discrete Fourier transform (DFT) on each discrete $N\times T$ spatio-temporal plane of the embeddings $\mathbf{X}^{\mathcal{G}}_t$ and obtain the frequency input $\mathcal{X}^{\mathcal{G}}_t:=\operatorname{DFT}(\mathbf{X}^{\mathcal{G}}_t) \in \mathbb{C}^{NT\times d}$. % to learn a Fourier graph $\mathcal{G}=(\mathcal{X},\mathcal{S})$ for adaptively inferring $G$ in the Fourier space.

Next, we feed $\mathcal{X}^{\mathcal{G}}_t$ to $K$-layer FourierGNN (denoted as $\Psi_K$) to perform graph convolutions for capturing the spatiotemporal dependencies simultaneously in Fourier space. 
%Then, we perform 2D inverse Fourier transform to generate representations $\mathbf{X}_{\Psi}:=\operatorname{IDFT}(\Psi_K(\mathcal{X}))\in \mathbb{R}^{N\times T\times d}$ in the time domain. 
The resulting representations $\mathcal{Y}^{\mathcal{G}}_t:=\Psi_K(\mathcal{X}^{\mathcal{G}}_t)$ are then transformed back to the time domain using inverse Fourier transform, which yields $\mathbf{Y}^{\mathcal{G}}_t:=\operatorname{IDFT}(\mathcal{Y}^{\mathcal{G}}_t)\in \mathbb{R}^{NT\times d}$.
Finally, we use a feed-forward network (FFN) (see Appendix \ref{subsec:es} for more details) to project $\mathbf{Y}^{\mathcal{G}}_t$ onto $\tau$ future steps, resulting in $\hat{Y}_t \in \mathbb{R}^{N\times \tau}$.
%As show in Fig. \ref{fig:model_fig}, EV-FGN contains a sequence of $K$ FGSO layers in a well-designed connection with each parameterized FGSO $\mathcal{S}\in\mathbb{C}^{d\times d}$ and sums all outputs of $K$ layers as the final output $\Psi_K(\mathcal{X})$.

%To make predictions in time domain, we perform 2D inverse Fourier transform to generate representations $\mathbf{X}_{\Psi}:=\operatorname{IDFT}(\Psi_K(\mathcal{X}))\in \mathbb{R}^{N\times T\times d}$ in the time domain. The representation is then fed to two-layer feed-forward networks (FFN, see details in Appendix \ref{subsec:es}) parameterized with weights and biases denoted as $\phi_{ff}$ to make predictions for future $\tau$ steps $\hat{X} \in \mathbb{R}^{N\times \tau}$ by one forward procedure. The L2 loss function for multi-step forecasting can be formulated as:%$$W \in \mathbb{R}^{T*d\times\tau}$ and bias $b \in \mathbb{R}^{N\times \tau}$
%\begin{equation}
%    \mathcal{L}(\hat{X};X;\Theta) = \sum_{t}\left\Vert \hat{X}_{t+1:t+\tau}-X_{t+1:t+\tau} \right\Vert_2^2
%    %= \sum_{t}\left\Vert \operatorname{F}(X^{t-T:t};\mathcal{G};\Theta)-X^{t+1:t+\tau}\right\Vert_2^2
%\end{equation}%=$\Theta$
%with parameters $\Theta=\{E_\phi,\phi_{ff},\Psi_K\}$. % and the groudtruth $X_{t+1:t+\tau}\subset\mathbb{X}$.

==> 3_method_v2.tex <==
%$x_t^{(n)} \in \mathbb{R}^1$ --> $\bm{x}_t \in \mathbb{R}^{N}$ --> $X_t \in \mathbb{R}^{N \times T}$  -->  $\mathcal{G}({X^\mathcal{G}_t},{A_t^\mathcal{G}})$ --> $\mathcal{G}({\mathbf{X}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> $\mathcal{G}({\mathcal{X}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> Shift Operator (AXW) --> $\mathcal{G}({\mathcal{Y}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> $\mathcal{G}({\mathbf{Y}^\mathcal{G}_t},{{A}_t^\mathcal{G}})$ --> 
%$ \hat{Y}_t \in \mathbb{R}^{N \times \tau}$.
\section{Problem Definition}
%Let us denote an entire multivariate time series (MTS) dataset as $\mathbb{X} \in \mathbb{R}^{N\times L}$ where $N$ is the number of variables and $L$ is the number of timestamps of the whole dataset. 
%Under the rolling setting, the time-series inputs are defined as averagely sampled lookback windows of length $T$, i.e., $\{X|X\subset\mathbb{X},X\in\mathbb{R}^{N\times T}\}$. 
Given the multivariate time series input, i.e., the lookback window $X_t=[\bm{x}_{t-T+1},...,\bm{x}_t]\in\mathbb{R}^{N\times T}$ at timestamps $t$ with the number of variables $N$ and the lookback window size $T$, where $\bm{x} \in \mathbb{R}^{N}$ denotes the multivariate values of $N$ distinct series at timestamp $t$, then the \textit{multivariate time series forecasting} task is to predict the next $\tau$ timestamps $Y_t=[{\bm{x}}_{t+1}, ..., {\bm{x}}_{t+\tau}]\in \mathbb{R}^{N \times \tau}$ based on the historical $T$ observations $X_t=[\bm{x}_{t-T+1},...,\bm{x}_t]$. The forecasting process can be given by:
% \begin{equation}\label{eq:problem_define}
%     \hat{\bm{x}}_{t+1},...,\hat{\bm{x}}_{t+\tau} = {F_{\theta}}(\bm{x}_{t-T+1},...,\bm{x}_t))
% \end{equation}
\begin{equation}\label{eq:problem_define}
   \hat{Y}_t  = {F_{\theta}}(X_t) = {F_{\theta}}([\bm{x}_{t-T+1},...,\bm{x}_t])
\end{equation}
where $\hat{Y}_t$ are the predicted results; the forecasting function is denoted as $F_\theta$ parameterized by $\theta$.
In practice, many MTS forecasting models usually leverage a \textit{graph network} (assume parameterized by $\theta_g$) to learn the spatial dynamics and a \textit{temporal network} (assume parameterized by $\theta_t$)  to learn the temporal dependencies, respectively \cite{zonghanwu2019, Cao2020,Bai2020nips,wu2020connecting,tampsgcnets2022}. Thus, the original definition of Equation (\ref{eq:problem_define}) can be rewritten to:
% \begin{equation}\label{eq:problem_define_gt}
%     \hat{\bm{x}}_{t+1},...,\hat{\bm{x}}_{t+\tau} = {F_{{\theta_g},{\theta_t}}}(\bm{x}_{t-T+1},...,\bm{x}_t)
% \end{equation}
\begin{equation}\label{eq:problem_define_gt}
    \hat{Y}_t  = {F_{\theta}}(X_t) = F_{\theta_g,\theta_t}([\bm{x}_{t-T+1},...,\bm{x}_t])
\end{equation}
where original parameters $\theta$ are exposed to the parameters of the graph network and the temporal network ${\theta_g}, {\theta_t}$ to make predictions based on the learned spatial-temporal dependencies.
%{
%\color{red}
%In the following section, we detnote the lookback window at timestamp $t$ as $X_t$, and the horizon window as $Y_t$ for brevity. 
%}

% $F_{\theta_g}$ with parameters $\theta_g$ for spatial correlations and a temporal network $F_{\theta_t}$ with parameters $\theta_t$ for temporal dependencies. Subsequently, a forecasting function $F_{\theta_f}$ with parameters $\theta_f$ is applied to make predictions based on the learned spatial-temporal dependencies. As a result, the forecasting problem is formulated as follows:
% \begin{equation}
%     \hat{X}_{t+1},...,\hat{X}_{t+\tau} = {F_{\theta_f}}((F_{\theta_g},F_{\theta_s})(X_{t-T},...,X_t))
% \end{equation}
%where $\operatorname{F}$ is the forecasting function and $\Theta$ is the learnable parameters of the forecasting function.


\section{Methodology}
In this section, we elaborate on our new framework: First, we start with our pure graph formulation with a novel data structure for MTS forecasting
in Section \ref{sec:method_pure_graph_form}. Then, we illustrate the proposed neural architecture, Fourier Graph Neural Network (FourierGNN), for this formulation in Section \ref{sec:method_fouriergnn}. Besides, we 
present theoretical analysis towards FourierGNN to demonstrate its validity.

\subsection{The Pure Graph Formulation}\label{sec:method_pure_graph_form}
To overcome the uncertain compatibility of the graph network and the temporal network as aforementioned in Section \ref{sec:intro}, and learn united spatiotemporal dynamics, we introduce a \textit{pure} graph formulation that refines Equation (\ref{eq:problem_define_gt}) by introducing a novel data structure, \textit{hypervariate graph}, for time series.
% In this paper, our goal is to learn an united view of spatiotemporal dynamics simultaneously and model the interdependencies between variables and their evolution over time, to this end, we build a hypervariate graph $\mathcal{G}=(X,A)$ attributed to each $X$ and further formulate the problem of MTS forecasting on the hypervariate graph. 
 \begin{myDef}[\textbf{Hypervariate Graph}]
\label{hypervariate_graph}
    Given a multivariate time series input $X_t \in \mathbb{R}^{N \times T}$ of $N$ variables over $T$ timestamps, we construct a hypervariate graph of $NT$ nodes, $\mathcal{G}_t=({X}^{\mathcal{G}}_t, {A}^{\mathcal{G}}_t)$, by regarding each element of $X_t$ 
    %(regardless of variables or timestamps)
    as one node of $\mathcal{G}_t$ such that ${X}^{\mathcal{G}}_t \in \mathbb{R}^{NT \times 1}$ stand for the node features and ${A}^{\mathcal{G}}_t \in \mathbb{R}^{NT \times NT}$ is the adjacency matrix.
    % variable at each timestamp is represented by a node in the graph, with $X\in \mathbb{R}^{NT}$ representing the nodes and $A \in \mathbb{R}^{(NT) \times (NT)}$ being the adjacency matrix. We refer to the graph $\mathcal{G}$ as a hypervariate graph.
\end{myDef}
 The hypervariate graph $\mathcal{G}_t$ contains $NT$ nodes that represent values of each variable at each timestamp in $X_t$. %and $A^{\mathcal{G}}_t \in \mathbb{R}^{NT \times NT}$ represents the connection structure of $\mathcal{G}.
 Since the prior graph structure is usually unknown in most scenarios, and each element of $X_t$ are spatially or temporally correlated with each other, we assume all nodes in the hypervariate graph $\mathcal{G}_t$ are fully-connected, in order to learn a joint spatiotemporal representation. More analysis about the hypervariate graph can be seen in Appendix \ref{analysis_hypervariate_graph}.
 Accodingly,
 %given the observed values of previous $T$ steps at timestamp $t$, i.e., $X_{t-T+1},...,X_{t}\in \mathbb{R}^{N\times T}$, 
 %the task of \textit{multivariate time series forecasting} is to predict the values of $N$ variables for next $\tau$ steps denoted as $\hat{X}_{t+1},...,\hat{X}_{t+\tau}\in \mathbb{R}^{N\times \tau}$ on the hypervariate graph $\mathcal{G}$. 
 %Thus, the problem formulation is modified as follows:%according to the learned spatial-temporal dependencies 
 we reformulate \textit{multivariate time series forecasting} into the predictions on the hypervariate graphs and rewrite the equation (\ref{eq:problem_define_gt}) as:
 %on the hypervariate graph $\mathcal{G}_t=({X}^{\mathcal{G}}_t, {A}^{\mathcal{G}}_t)$ and the problem formulation is modified as follows:
\begin{equation}
    \hat{Y}_t =F_{\theta_\mathcal{G}}({X^\mathcal{G}_t},{A_t^\mathcal{G}})
\end{equation}
where $\theta_\mathcal{G}$ stand for the parameters of hypervariate graphs,
instead of  being split into separate ${\theta_g}$ and ${\theta_t}$ for two networks in Equation (\ref{eq:problem_define_gt}).
With such a formulation, we can view the spatial dynamics and the temporal dependencies with an united structure, which benefits modeling the real-world spatiotemporal inter-dependencies.


%where $\operatorname{F}$ is the forecasting model with parameters $\Theta$. 

\subsection{FourierGNN}\label{sec:method_fouriergnn}
%With the hypervariate graph $\mathcal{G}$, we can view spatiotemporal dynamics as a whole, which facilitates the modeling of intricate interdependencies between various variables and timestamps. 
%To learn the united spatiotemporal dynamics, we perform graph convolutions on $\mathcal{G}$.
%Nevertheless, 
Though the pure graph formulation enhances spatiotemporal modeling, 
the order and size of hypervariate graphs increase with the number of variables $N$ and the length of window $T$, which makes classic graph networks (e.g., GCN~\cite{}, GAT~\cite{}, etc) computationally expensive (usually quadratic complexity) and suffer from optimization difficulties to obtaining accurate hidden node representations~\cite{}. 
In this regard, we propose an efficient and effective method, FourierGNN, for the pure graph formulation. Specifically, we first elaborate on our proposed built-in component, Fourier Graph Shift Operator (FGSO) in Section \ref{FGSO}; then we illustrate the stacked architecture of FourierGNN with FGSOs 
in Section \ref{FGNN}; finally, we present the overall pipeline using FourierGNN for forecasting in Section \ref{architecture}.



% Specifically, in \ref{FGSO} we design a replacement of classic graph convolution units in Fourier space (i.e., FGSO), and then implement graph convolutions by stacking FGSOs in Fourier space (i.e., FourierGNN) in \ref{FGNN}. Finally, we introduce our overall network architecture based on FourierGNN for MTS forecasting in \ref{architecture}.

%FourierGNN we introduce  shift operator, in Section XXX, 
%built on operator, we illustarte archir3ecture, Figure ref{},
%we theoreatical analysis  
%4.2.1 shift operator (including inference for FGSO)
%4.2.2 overall architecture (current 4.2.1 + partial current 4.2.3)
%4.2.3 model analysis (prove in 4.2.3)

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/FourierGNN_model_1.pdf}
    \caption{\textcolor{red}{The network architecture of our proposed model}. Given an input $X\in \mathbb{R}^{N \times T}$, we 1) embed $X$ into $\mathbf{X}\in \mathbb{R}^{N\times T \times d}$; 2) transform $\mathbf{X}$ to Fourier space $\mathcal{X} \in \mathbb{C}^{N \times T \times d}$ by 2D DFT on the discrete N × T spatial-temporal space; 3) perform graph convolutions in Fourier space by conducting multiplication of FGSO $\mathcal{S}$ and $\mathcal{X}$ in the $K$-layer FourierGNN; 4) transform the output of FourierGNN to time domain $\mathbf{X}_{\Psi}\in \mathbb{R}^{N\times T \times d}$ by 2D IDFT; 5) generate $\tau$-step predictions $\hat{X} \in \mathbb{R}^{N \times \tau}$ via feeding $\mathbf{X}_{\Psi}$ to a two-layer feed-forward network.}
    \label{fig:model_fig}
\end{figure}

\subsubsection{Fourier Graph Shift Operator}\label{FGSO}
According to the discrete signal processing on graphs \cite{SandryhailaM13}, a graph shift operator (GSO) is defined as a general family of operators which enables the diffusion of information over graph structures~\cite{GamaRB20,Dasoulas2021}.
%Note that the supra-graph $n=NT$.
%\TODO{
%Definition 2 --> 
%(4) --> 
%However, Equation (4) has quadratic complexity due to S X ~ n, which brings potential challenges in our pure graph formulation. 
%Thus, we define a Fourier Graph shift operator to solve this problem. 
%-->
%Definition 3,  $\mathcal{S}$ = 
%-->
%}
\begin{myDef}[\textbf{Graph Shift Operator}]
\label{def:gso}
Given a graph $G$ with $n$ nodes, a matrix $S\in\mathbb{R}^{n\times n}$ is called a \textit{Graph Shift Operator} (GSO) if it satisfies $S_{ij}=0$ if $i\neq j$ and nodes $i,j$ are not connected.
\end{myDef}
Usually, the graph shift operator includes the adjacency, Laplacian matrices and their according normalization as instances of its class~\cite{Dasoulas2021}. 
Thus, given the graph $G$ attributed to $X\in\mathbb{R}^{n\times d}$ and the graph shift operator $S$, %a general form of spatial-based graph convolution is defined as
we can express the classic graph convolution~\cite{KipfW17} as:
%a general form of graph convolution~\cite{KipfW17} is defined as
\begin{equation}
\label{equ:graph_covolution}
    O({X}):=S{X}{W}
\end{equation}
with the parameter matrix ${W}\in\mathbb{R}^{d\times d}$. However, Equation (\ref{equ:graph_covolution}) has quadratic complexity with $n$, which brings potential computational challenges in our pure graph formulation ($n$ corresponds to $NT$ in our formulation). Therefore, to solve this problem, we define a Fourier Graph Shift Operator.
%Regarding $S$ as $n\times n$ scores, we can define a matrix-valued kernel $\kappa: [n]\times [n] \xrightarrow{} \mathbb{R}^{d\times d}$ with $\kappa[i,j]=S_{ij}\circ {W}$, where $[n]=\{1,2,\cdots,n\}$.
\begin{myDef}[\textbf{Fourier Graph Shift Operator}]
\label{def:fgso}
Given a graph $G=(X, S)$ with input $X\in\mathbb{R}^{n\times d}$ and GSO $S \in\mathbb{R}^{n\times n}$, and the weight matrix $W\in\mathbb{R}^{d\times d}$, we define a matrix-valued kernel $\kappa: [n]\times [n] \xrightarrow{} \mathbb{R}^{d\times d}$ with $\kappa[i,j]=S_{ij}\circ {W}$, where $[n]=\{1,2,\cdots,n\}$. Then, we define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{d \times d}$ as a Fourier graph shift operator (FGSO), where $\mathcal{F}$ denotes DFT.
\end{myDef} 
Accordingly, with the Fourier graph shift operator (FGSO), according to the convolution theorem~\cite{1970An} (see Appendix \ref{convolution_theorem_appendix}), the multiplications between $\mathcal{F}(X)$ and FGSO $\mathcal{S}$ in Fourier space can be written as:
\begin{equation}\label{equ:fgso}
    (\mathcal{F}(X)\mathcal{S})[i]=(\mathcal{F}(X)\mathcal{F}(\kappa))[i] = \sum_{j=1}^n {X}[j]\kappa[i-j] \quad\quad   \forall i \in [n].
\end{equation}
In the special case of the Green's kernel $\kappa[i,j]=\kappa[i-j]$, we can rewrite the right part of above equation as follows:
\begin{equation}\label{equ:kernel_summation}
    \sum_{j=1}^n {X}[j]\kappa[i-j]=\sum_{j=1}^n {X}[j]\kappa[i,j]  \quad\quad   \forall i \in [n].
\end{equation}
Then, we extend the matrix-valued kernel $\kappa[i,j]=S_{ij}\circ {W}$ to the right part of Equation (\ref{equ:kernel_summation}), and obtain $\sum_{j=1}^n {X}[j]\kappa[i,j]=\sum_{j=1}^n S_{ij}{X}[j]W=(SXW)[i]$. Finally, combining Equation (\ref{equ:fgso}), we can get the following formula:
\begin{equation}
    \mathcal{F}(X)\mathcal{F}(\kappa) = SXW
\end{equation}
Therefore, the matrix multiplication between the DFT of input $\mathcal{F}(X)$ and the FGSO $\mathcal{F}(\kappa)$ in Fourier space is equivalent to the classic graph convolution on $X$ in the time domain. 

This

Compared with the time domain,

%we reformulate the graph convolution as:
%\begin{equation}
%    \label{equ:fgso}
%    \mathcal{F}(SXW)=\mathcal{F}(X)\times_n\mathcal{F}(\kappa)
%\end{equation}
%where we define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).
%where $\mathcal{F}$ denotes DFT, satisfies $\kappa[i,j]=\kappa[i-j]$, and $\times_n$ is matrix multiplication on dimensions except that of $n$. We define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).

%Regarding $S$ as $n\times n$ scores, we can define a matrix-valued kernel $\kappa: [n]\times [n] \xrightarrow{} \mathbb{R}^{d\times d}$ with $\kappa[i,j]=S_{ij}\circ {W}$, where $[n]=\{1,2,\cdots,n\}$. 

%Then the graph convolution can be viewed as a kernel summation:
%\begin{equation}
%    O({X})[i]=\sum_{j=1}^n {X}[j]\kappa[i,j]  \quad\quad   \forall i \in [n].
%\end{equation}
%In the special case of the Green's kernel $\kappa[i,j]=\kappa[i-j]$, we can rewrite the above equation as:
%\begin{equation}\label{equ:kernel_summation}
%    O({X})[i]=\sum_{j=1}^n {X}[j]\kappa[i-j]=(X*\kappa)[i]  \quad\quad   \forall i \in [n].
%\end{equation}
%with $X*\kappa$ denotes the convolution of discrete sequences $X$ and $\kappa$. According to the convolution theorem~\cite{1970An} (see Appendix \ref{convolution_theorem_appendix}), we can rewrite the graph convolution of Equation (\ref{equ:kernel_summation}) as:
%\begin{equation}
%\label{equ:fno}
%O(X)(i) = \mathcal{F}^{-1}\left(\mathcal{F}(X)\mathcal{F}(\kappa)\right)(i)\quad\quad  \forall i \in [n].
%\end{equation}
%where $\mathcal{F}$ and $\mathcal{F}^{-1}$ denote the Discrete Fourier Transform (DFT) and the inverse DFT, respectively. 
%The multiplication in the Fourier space is a lower-complexity computation compared to the graph convolution, and DFT can be efficiently implemented by the fast Fourier transform (FFT). %In the following, we define the Fourier Graph Shift Operator.
%\begin{myDef}[\textbf{Fourier Graph Shift Operator}]
%\label{def:fgso}
%Given a graph $G=(X, S)$ with input $X\in\mathbb{R}^{n\times d}$ and GSO $S \in\mathbb{R}^{n\times n}$ and the weight matrix $W\in\mathbb{R}^{d\times d}$, we reformulate the graph convolution as:
%\begin{equation}
%    \label{equ:fgso}
%    \mathcal{F}(SXW)=\mathcal{F}(X)\times_n\mathcal{F}(\kappa)
%\end{equation}
%where we define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).
%where $\mathcal{F}$ denotes DFT, satisfies $\kappa[i,j]=\kappa[i-j]$, and $\times_n$ is matrix multiplication on dimensions except that of $n$. We %define $\mathcal{S}:=\mathcal{F}(\kappa)\in\mathbb{C}^{n \times d \times d}$ as a Fourier graph shift operator (FGSO).
%\end{myDef} 
%In particular, turning to our case of the fully-connected hypervariate graph $\mathcal{G}$ with a fully-connected GSO $A^{\mathcal{G}}_t\in\{1\}^{n \times n}$, it yields the space-invariant kernel $\kappa[i,j]=A^{\mathcal{G}}_{ij}\circ{W}=W$ and $\mathcal{F}(A^{\mathcal{G}}_tX^{\mathcal{G}}_tW)=\mathcal{F}(X^{\mathcal{G}}_t)\mathcal{F}(\kappa)$. Accordingly, we can parameterize FGSO $\mathcal{A}^{\mathcal{G}}_t$ with a complex-valued matrix $\mathbb{C}^{d \times d}$ which is frequency-invariant and is computationally low costly compared to a varying kernel resulting a parameterized matrix of $\mathbb{C}^{n \times d\times d}$. 
%Furthermore, we generalize Definition \ref{def:fgso} to 2D discrete space, i.e., from $[n]$ to $[N]\times[T]$, corresponding to the finite discrete spatio-temporal space of multivariate time series. 
%See Appendix \ref{explanation} for more explanations on the frequency-invariant FGSO. 
%and the extension to 2D domain.

\textbf{Remarks}. 
%Compared with FGSO and FNO, frequency-invariant FGSO has several advantages. 
Frequency-invariant FGSO has several advantages. 
Assume a graph with $n$ nodes and the embedding dimension $d$ ($d\leq n$). 1) \textit{Efficiency}: the time complexity of frequency-invariant FGSO is $O(nd\operatorname{log}n+nd^2)$ for DFT, IDFT and the matrix multiplication compared with that of $O(n^2d+nd^2)$ on a GSO. 2) \textit{Scale-free parameters}: frequency-invariant FGSO strategically shares $O(d^2)$ parameters for each node and the parameter volume is agnostic to the data scale.
%, while the parameter count of FNO is $O(nd^2)$.% More analyses are given in Appendix \ref{proof_proposition}.

\subsubsection{Fourier Graph Neural Networks}\label{FGNN}

\TODO{ 
The specific design of  FourierGNN is by stacking multiple layers of  GGSOs with learnable layers. Specifically, we can define FourierGNN as: 

$ \operatorname{FourierGNN}(X, \mathcal{S}) = \mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\times_n\mathcal{S}_{0:k}\right)\quad s.t.\  \mathcal{S}_{0:k}=\mathcal{S}_0\times_n\cdots\mathcal{S}_{K-1}\times_n\mathcal{S}_{K} $
}
where $S =$






Graph filters as core operations in graph signal processing are linear transformations expressed as polynomials of the graph shift operator~\cite{isufi2021edgenets,MateosSMR19} and can be used to exactly model graph convolutions and capture multi-order diffusion on graph structures~\cite{SegarraMMR17}. 
%\begin{equation}
%    Z_k = S^{K:0} Z_{k-1} W^{K}
%\end{equation}
The $K$-order graph filters $H_K$ are defined as follows~\cite{isufi2021edgenets,SegarraMMR17}:
%graph filter-->edge varying graph filter
\begin{equation}
    H_{K} X= S_0X+S_1S_0X+...+S_KS_{K-1}...S_0X=\sum_{k=0}^{K}\left ( \prod_{k'=0}^{k} S_{k'} \right ) X
\end{equation}
where $S_0$ denotes the identity matrix, $\{S_k\}_{k=1}^K$ is a collection of $K$ GSOs sharing the sparsity pattern of $S$, and $S_k\in\mathbb{R}^{n\times n}$ corresponds to the $k$-th diffusion step.
%\begin{equation}
%    X^(k) = S_K X^(k-1)
%\end{equation}
To capture the time-varying counterparts, we design edge-variant graph filters $H_{K}^{EV}$ by adopting different weights to measure the information of different neighbors in each diffusion order~\cite{isufi2021edgenets}:
%the edge-variant graph filters $H_{EV}$ are defined as follows~\cite{isufi2021edgenets,SegarraMMR17}: given GSO $S\in\mathbb{R}^{n\times n}$ corresponding to a graph with $n$ nodes,
\begin{equation}
    H_{K}^{EV} X = S_0 X W_0+S_1(S_0XW_0)W_1+...+S_K(S_{K-1}...(S_0XW_0)...W_{K-1})W_K %=\sum_{k=0}^{K}S_{k:0}
\end{equation}
%\begin{equation}
%   X_K= \Phi_K X_{K-1} W_{K}
%\end{equation}
%where $S_0$ denotes the identity matrix, $\{S_k\}_{k=1}^K$ is a collection of $K$ edge-weighting GSOs sharing the sparsity pattern of $S$, and $S_k\in\mathbb{R}^{n\times n}$ corresponds to the $k$-th diffusion step. 
where $W_{k} \in \mathbb{R}^{d \times d}$ is a parameter matrix that affords flexibility to process different features with different filter parameters.
The edge-variant graph filters are proved effective to yield a highly discriminative model and lay the foundation for the unification of GCNs and GATs~\cite{isufi2021edgenets}. We further extend Equation (\ref{equ:fgso}) to $H^{EV}_K$ and reformulate the multi-order graph convolution in a recursive form.
%, where we omit the weight $W$ for conciseness.
%\prod_{i=1}^k S_{i}
\begin{myPro}%[\textbf{Equivalence}]
\label{pro:filter}
Given a graph input $X\in\mathbb{R}^{n\times d}$, the $K$-order graph convolution under the edge-variant graph filter $H^{EV}_K$
%=\sum_{k=0}^{K}A_{k:0}$ with $\{A_k\in\mathbb{R}^{n\times n}\}_{k=0}^K$ 
is reformulated as follows:
    \begin{equation} 
    \label{equ:fgso_filter}
        H_K^{EV}X=\mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\times_n\mathcal{S}_{0:k}\right)\quad s.t.\  \mathcal{S}_{0:k}=\mathcal{S}_0\times_n\cdots\mathcal{S}_{K-1}\times_n\mathcal{S}_{K}
    \end{equation}
where $\mathcal{S}_k\in\mathbb{C}^{n\times d\times d}$ is the $k$-th FGSO satisfying $\mathcal{F}(S_k {X} W_k)=\mathcal{F}({X})\times_n\mathcal{S}_k$, $\mathcal{S}_0$ is the identity matrix, and $\mathcal{F}$ and $\mathcal{F}^{-1}$ denote the discrete Fourier transform and its reverse, respectively.
\end{myPro}
Proposition \ref{pro:filter} proved in Appendix \ref{sec:filter} states that we can rewrite the multi-order graph convolution corresponding to $H_K^{EV}$ as a summation of a recursive multiplication of individual FGSO in Fourier space. Corresponding to our case of the hypervariate graph $\mathcal{G}$, we can similarly adopt $K$ frequency-invariant FGSOs and parameterize each FGSO $\mathcal{A}_k$ with a complex-valued matrix $\mathbb{C}^{d\times d}$. This saves a large amount of computation costs and results in a concise form:
\begin{equation} 
    \label{equ:fgso_filter_2}
        H_K^{EV}X=\mathcal{F}^{-1}\left(\sum_{k=0}^{K}\mathcal{F}(X)\mathcal{A}_{0:k}\right)\quad s.t.\  \mathcal{A}_{0:k}=\prod_{i=0}^k\mathcal{A}_i
    \end{equation}
The recursive composition has a nice property that $\mathcal{A}_{0:k}=\mathcal{A}_{0:k-1}\mathcal{A}_k$, which inspires us to design a complex-valued feed forward network with $\mathcal{A}_k$ being the complex weights for the $k$-th layer. However, both the FGSO and edge-variant graph filter are linear transformations, limiting the capability of modeling non-linear information diffusion on graphs. Following by the convention in GNNs, we introduce the non-linear activation and biases to reformulate the $k$-the layer as follows: 
\begin{equation}
    \label{equ:layer}
    \mathcal{X}_k = \sigma(\mathcal{X}_{k-1}\mathcal{A}_k+b_k)
\end{equation}
with the complex weight $\mathcal{A}_k \in \mathbb{C}^{d\times d}$, biases $b_k \in \mathbb{C}^{d}$ and the activation function $\sigma$. Accordingly, we design a Fourier graph neural network (FourierGNN) in Fourier space according to Equations (\ref{equ:fgso_filter}) and (\ref{equ:layer}), as shown in Fig. \ref{fig:model_fig}. Accordingly, the $K$-layer FourierGNN $\Psi_K$ is formulated:
\begin{equation}
    \Psi_K(\mathcal{X})=\sum_{k=0}^K \mathcal{X}_{k} \quad s.t.\ \mathcal{X}_k=\sigma(\mathcal{X}_{k-1}\mathcal{A}_k+b_k)
\end{equation}
where $\mathcal{X}_0:=\mathcal{F}(\mathbf{X})$, $\{\mathcal{A}_k\in\mathbb{C}^{d\times d}\}_{k=1}^K$ and $\{b_{k}\in\mathbb{C}^{d}\}_{k=1}^K$ are complex-valued parameters. 
%The frequency output $\Psi_K(\mathcal{X})$ is then transformed via IDFT, followed with feed forward networks (see Appendix \ref{subsec:es} for more details) to make multi-step forecasting in the time domain.

\textbf{Remarks}. FourierGNN efficiently learns edge- and neighbor-dependent weights to compute multi-order graph convolutions on one fly in Fourier space with scale-free parameter volume. For $K$ iterations of graph convolutions, GCNs have a general time complexity of $O(Kn^2d+Knd^2)$, 
%and FNO needs $O(Knd\operatorname{log}n+Knd^2)$, 
and FourierGNN achieves a time complexity of $O(nd\operatorname{log}n+Knd^2+Knd)$. 
FourierGNN 
%saves time costs from FNO in Fourier transforms and 
is much more efficient than GCNs, especially in our case with $n=NT$ for a given raw input $X^{\mathcal{G}}_t\in\mathbb{R}^{N\times T}$. 
See Appendix \ref{compares} for more details about the relations and differences between FourierGNN with other neural networks.
%FNO, adaptive FNO, and GNNs.

% to connect all observed values $\{x_{it}\}$ among variables and timestamps
\subsubsection{Overall Architecture} \label{architecture}
\label{sec:ovarc}
The overall architecture of our model is illustrated in Fig. \ref{fig:model_fig}. Given the MTS input data $X_t \in \mathbb{R}^{N\times T}$, first we construct a fully-connected hypervariate graph $\mathcal{G}=(X^{\mathcal{G}}_t, A^{\mathcal{G}}_t)$ with $X^{\mathcal{G}}_t \in \mathbb{R}^{NT \times 1}$. Then, we embed the data into embeddings $\mathbf{X}^{\mathcal{G}}_t \in \mathbb{R}^{NT\times d}$ by assigning a $d$-dimension vector for each node using an embedding matrix $E_\phi\in\mathbb{R}^{1\times d}$, i.e., $\mathbf{X}^{\mathcal{G}}_t=X^{\mathcal{G}}_t \times E_\phi$. 
%Instead of directly learning the huge embedding matrix, we introduce two small parameter matrices: 1) a variable embedding matrix $\phi_v\in\mathbb{R}^{N\times 1\times d}$, and 2) a temporal embedding matrix $\phi_u\in\mathbb{R}^{1\times T\times d}$ to factorize $\Phi$, i.e., $\Phi=\phi_v\times \phi_u$. 

Subsequently, we perform discrete Fourier transform (DFT) on each discrete $N\times T$ spatio-temporal plane of the embeddings $\mathbf{X}^{\mathcal{G}}_t$ and obtain the frequency input $\mathcal{X}^{\mathcal{G}}_t:=\operatorname{DFT}(\mathbf{X}^{\mathcal{G}}_t) \in \mathbb{C}^{NT\times d}$. % to learn a Fourier graph $\mathcal{G}=(\mathcal{X},\mathcal{S})$ for adaptively inferring $G$ in the Fourier space.

Next, we feed $\mathcal{X}^{\mathcal{G}}_t$ to $K$-layer FourierGNN (denoted as $\Psi_K$) to perform graph convolutions for capturing the spatiotemporal dependencies simultaneously in Fourier space. 
%Then, we perform 2D inverse Fourier transform to generate representations $\mathbf{X}_{\Psi}:=\operatorname{IDFT}(\Psi_K(\mathcal{X}))\in \mathbb{R}^{N\times T\times d}$ in the time domain. 
The resulting representations $\mathcal{Y}^{\mathcal{G}}_t:=\Psi_K(\mathcal{X}^{\mathcal{G}}_t)$ are then transformed back to the time domain using inverse Fourier transform, which yields $\mathbf{Y}^{\mathcal{G}}_t:=\operatorname{IDFT}(\mathcal{Y}^{\mathcal{G}}_t)\in \mathbb{R}^{NT\times d}$.
Finally, we use a feed-forward network (FFN) (see Appendix \ref{subsec:es} for more details) to project $\mathbf{Y}^{\mathcal{G}}_t$ onto $\tau$ future steps, resulting in $\hat{Y}_t \in \mathbb{R}^{N\times \tau}$.
%As show in Fig. \ref{fig:model_fig}, EV-FGN contains a sequence of $K$ FGSO layers in a well-designed connection with each parameterized FGSO $\mathcal{S}\in\mathbb{C}^{d\times d}$ and sums all outputs of $K$ layers as the final output $\Psi_K(\mathcal{X})$.

%To make predictions in time domain, we perform 2D inverse Fourier transform to generate representations $\mathbf{X}_{\Psi}:=\operatorname{IDFT}(\Psi_K(\mathcal{X}))\in \mathbb{R}^{N\times T\times d}$ in the time domain. The representation is then fed to two-layer feed-forward networks (FFN, see details in Appendix \ref{subsec:es}) parameterized with weights and biases denoted as $\phi_{ff}$ to make predictions for future $\tau$ steps $\hat{X} \in \mathbb{R}^{N\times \tau}$ by one forward procedure. The L2 loss function for multi-step forecasting can be formulated as:%$$W \in \mathbb{R}^{T*d\times\tau}$ and bias $b \in \mathbb{R}^{N\times \tau}$
%\begin{equation}
%    \mathcal{L}(\hat{X};X;\Theta) = \sum_{t}\left\Vert \hat{X}_{t+1:t+\tau}-X_{t+1:t+\tau} \right\Vert_2^2
%    %= \sum_{t}\left\Vert \operatorname{F}(X^{t-T:t};\mathcal{G};\Theta)-X^{t+1:t+\tau}\right\Vert_2^2
%\end{equation}%=$\Theta$
%with parameters $\Theta=\{E_\phi,\phi_{ff},\Psi_K\}$. % and the groudtruth $X_{t+1:t+\tau}\subset\mathbb{X}$.

==> rebuttal.tex <==
\textbf{review #G8af}



\textbf{review #ndBv}

\begin{table*}[h]
    \centering
    \caption{Long-term forecasting comparison. We set the lookback window size $L$ as 96 and the prediction length as $\tau \in \{96, 192, 336, 720\}$ except for traffic dataset whose prediction length is set as $\tau \in \{48, 96, 192, 336 \}$. The best results are in \textbf{bold} and the second best are \underline{underlined}. Full results of long-term forecasting are included in Appendix \ref{additional_long_term}.
    %For the METR-LA dataset, the input length is 24 and prediction length is \{24, 48, 96 and 128\}. For the Exchange dataset, the input length is 96 and prediction length is \{96, 192, 336 and 480\}.
    }
    %\resizebox{\textwidth}{24mm}{
    \scalebox{0.7}{
    \begin{tabular}{l c|c c|c c|c c| c c|c c |c c |c c}
    \toprule
    \toprule
       \multicolumn{2}{c|}{Models}  &\multicolumn{2}{c|}{FourierGNN} & \multicolumn{2}{c|}{PatchTST} & \multicolumn{2}{c|}{LTSF-Linear} & \multicolumn{2}{c|}{FEDformer} & \multicolumn{2}{c|}{Autoformer} & \multicolumn{2}{c|}{Informer} & \multicolumn{2}{c}{Reformer}\\
        \multicolumn{2}{c|}{Metrics}&MAE &RMSE &MAE &RMSE&MAE &RMSE&MAE &RMSE &MAE &RMSE &MAE &RMSE &MAE &RMSE\\
       \midrule
         \multirow{4}*{\rotatebox{90}{Weather}} &  96 & \textbf{0.032}& \textbf{0.071}& \underline{0.034}& \underline{0.074}& 0.040& 0.081&0.050 & 0.088&0.064 & 0.104& 0.101& 0.139&0.108 & 0.152\\
         & 192 & \textbf{0.040}& \textbf{0.081}& \underline{0.042}& \underline{0.084} & 0.048& 0.089& 0.051& 0.092& 0.061& 0.103&0.097 & 0.134& 0.147& 0.201\\
          &  336& \textbf{0.046}& \textbf{0.090}& \underline{0.049}& \underline{0.094}& 0.056& 0.098& 0.057& 0.100&0.059 &0.101 &0.115 & 0.155&0.154 & 0.203\\
         & 720 &\textbf{0.055} & \textbf{0.099}& \underline{0.056}& \underline{0.102}& 0.065& 0.106& 0.064 & 0.109&0.065 &0.110 &0.132 & 0.175&0.173 &0.228 \\
         \midrule
         \multirow{4}*{\rotatebox{90}{Exchange}} & 96 &\textbf{0.037} & \textbf{0.051}&0.039& \underline{0.052} &\underline{0.038} & \underline{0.052}& 0.050& 0.067& 0.050& 0.066& 0.066& 0.084& 0.126&0.146 \\
         & 192 & \textbf{0.050}& \textbf{0.067}&0.055& 0.074 & \underline{0.053}& \underline{0.069}& 0.064& 0.082& 0.063& 0.083& 0.068& 0.088& 0.147& 0.169\\
         & 336 & \textbf{0.062}& \textbf{0.082}&0.071& 0.093 & \underline{0.064}& \underline{0.085}& 0.080& 0.105& 0.075& 0.101& 0.093& 0.127& 0.157& 0.189\\
         & 720 & \textbf{0.088}& \textbf{0.110}&0.132& 0.166 & \underline{0.092}& \underline{0.116}& 0.151& 0.183& 0.150& 0.181& 0.117& 0.170& 0.166& 0.201\\
         \midrule
         \multirow{4}*{\rotatebox{90}{ETTh1}} &  96 & \textbf{0.061}& \textbf{0.087}& 0.065& 0.091& \underline{0.063}& \underline{0.089}& 0.072&0.096 &0.079 &0.105 &0.093 & 0.121&0.113 & 0.143\\
         & 192 & \textbf{0.065}& \textbf{0.091}& 0.069& \underline{0.094}& \underline{0.067}& \underline{0.094}& 0.076& 0.100&0.086 & 0.114& 0.103& 0.137& 0.120& 0.148\\
          &  336& \textbf{0.070}& \textbf{0.096}& \underline{0.073} & {0.099} & \textbf{0.070}& \underline{0.097}& 0.080& 0.105&0.088 & 0.119& 0.112& 0.145& 0.124& 0.155\\
         & 720 &\textbf{0.082} & \textbf{0.108}& \underline{0.087}& \underline{0.113}& \textbf{0.082}&\textbf{0.108} & 0.090& 0.116&0.102 & 0.136& 0.125& 0.157& 0.126& 0.155\\
         \midrule
         \multirow{4}*{\rotatebox{90}{ETTm1}} &  96 & \textbf{0.052}& \textbf{0.077}& \underline{0.055} & 0.082& \underline{0.055}& \underline{0.080}& 0.063&0.087 &0.081 &0.109 &0.070 & 0.096 &0.065 & 0.089\\
         & 192 & \textbf{0.057}& \textbf{0.083}& \underline{0.059}& \underline{0.085}& {0.060}& {0.087}& 0.068& 0.093 &0.083 & 0.112& 0.082& 0.107& 0.081& 0.108\\
          &  336& \textbf{0.062}& \textbf{0.089}& \underline{0.064} & \underline{0.091} & {0.065}& {0.093}& 0.075& 0.102&0.091 & 0.125& 0.090& 0.119& 0.100& 0.128\\
         & 720 &\textbf{0.069} & \textbf{0.096}& \underline{0.070}& \underline{0.097}& {0.072}&{0.099} & 0.081& 0.108&0.093 & 0.126 & 0.115& 0.149& 0.132& 0.163\\
         \bottomrule
         \bottomrule
    \end{tabular}
    }
    \label{tab:long_term}
    \vspace{-3mm}
\end{table*}



\textbf{review #ipTP}




\textbf{review #yaJh}
